Learned Video Compression for YUV 4:2:0 Content Using Flow-based Conditional Inter-frame Coding

This paper proposes a learning-based video compression framework for variable-rate coding on YUV 4:2:0 content. Most existing learning-based video compression models adopt the traditional hybrid-based coding architecture, which involves temporal prediction followed by residual coding. However, recent studies have shown that residual coding is sub-optimal from the information-theoretic perspective. In addition, most existing models are optimized with respect to RGB content. Furthermore, they require separate models for variable-rate coding. To address these issues, this work presents an attempt to incorporate the conditional inter-frame coding for YUV 4:2:0 content. We introduce a conditional flow-based inter-frame coder to improve the inter-frame coding efficiency. To adapt our codec to YUV 4:2:0 content, we adopt a simple strategy of using space-to-depth and depth-to-space conversions. Lastly, we employ a rate-adaption net to achieve variable-rate coding without training multiple models. Experimental results show that our model performs better than x265 on UVG and MCL-JCV datasets in terms of PSNR-YUV. However, on the more challenging datasets from ISCAS'22 GC, there is still ample room for improvement. This insufficient performance is due to the lack of inter-frame coding capability at a large GOP size and can be mitigated by increasing the model capacity and applying an error propagation-aware training strategy.

==> chapter/4-4_flow.tex <==
\begin{figure}[h]
\begin{center}
\begin{subfigure}{0.44\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \hspace{-2em}
    \includegraphics[width=0.9\linewidth]{figure/flow maps/ISCAS_Grand_Challenge_Validation5_ref_frame_step_332.png}
    \caption{reference frame}
    %\vspace{-1.2em}
    \label{fig:ref_frame}
\end{subfigure}%\hspace{-2em}%\hfill
\begin{subfigure}{0.44\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \includegraphics[width=0.9\linewidth]{figure/flow maps/ISCAS_Grand_Challenge_Validation5_gt_frame_step_332.png}
    \caption{current frame}
    %\vspace{-1.2em}
    \label{fig:gt_frame}
\end{subfigure}%\hspace{2em}

\begin{subfigure}{0.44\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \hspace{-2em}
    \includegraphics[width=0.9\linewidth]{figure/flow maps/ISCAS_Grand_Challenge_Validation5_flow_map_step_99.png}
    \caption{optical flow before overfit}
    %\vspace{-1.2em}
    \label{fig:flow_99}
\end{subfigure}%\hspace{-2em}%\hfill
\begin{subfigure}{0.44\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \includegraphics[width=0.9\linewidth]{figure/flow maps/ISCAS_Grand_Challenge_Validation5_flow_map_step_332.png}
    \caption{optical flow after overfit}
    %\vspace{-1.2em}
    \label{fig:flow_332}
\end{subfigure}%\hspace{2em}
\caption{\color{red}Optical flow comparison on the interlaced sequence.}
\label{fig:flow}
\end{center}
\vspace{-2.0em}
\end{figure}

==> chapter/6_Reference.tex <==
\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}
\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.


==> chapter/Z_Acknowledgment.tex <==

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.
